Propagation and Pitfalls: Reasoning-based Assessment of Knowledge Editing through Counterfactual Tasks

Current approaches of knowledge editing struggle to effectively propagate updates to interconnected facts. In this work, we delve into the barriers that hinder the appropriate propagation of updated knowledge within these models for accurate reasoning. To support our analysis, we introduce a novel reasoning-based benchmark -- ReCoE (Reasoning-based Counterfactual Editing dataset) -- which covers six common reasoning schemes in real world. We conduct a thorough analysis of existing knowledge editing techniques, including input augmentation, finetuning, and locate-and-edit. We found that all model editing methods show notably low performance on this dataset, especially in certain reasoning schemes. Our analysis over the chain-of-thought generation of edited models further uncover key reasons behind the inadequacy of existing knowledge editing methods from a reasoning standpoint, involving aspects on fact-wise editing, fact recall ability, and coherence in generation. We will make our benchmark publicly available.

==> prompts/alias_genereation.tex <==
\begin{figure*}[htbp]
\begin{lstlisting}
## Alias Generation

Human:

Generate aliases for the given entities. 
Here are some examples.

<example>

H: 
entity 1: Luis Fortuno
entity 2: Alejandro Garcia Padilla

A:
<response>

For entity 1 Luis Fortuno:
<entity1_alias1>Luis Guillermo Fortuno Burset</entity1_alias1>
<entity1_alias2>Luis G. Fortuno</entity1_alias2>
<entity1_alias3>Luis Fortuno</entity1_alias3>
<entity1_alias4>Luis G. Fortuno</entity1_alias4>
<entity1_alias5>Luis Guillermo Fortuno Burset</entity1_alias5>

For entity 2 Alejandro Garcia Padilla:
<entity2_alias1>Alejandro Javier Garcia Padilla</entity2_alias1>
<entity2_alias2>Garcia Padilla</entity2_alias2>
<entity2_alias3>Garcia-Padilla</entity2_alias3>
<entity2_alias4>Alejandro J. Garcia-Padilla</entity2_alias4>

</response>

</example>

Here are two new entities. 
Please generate their aliases.

entity 1: {{answer}}
entity 2: {{counterfactual answer}}

Assistant:
\end{lstlisting}
\caption{Alias Generation Prompt}
\label{fig:alias_generation}
\end{figure*}

==> prompts/atomic_facts.tex <==

\begin{figure*}[htbp]
\begin{lstlisting}
## Atomic Facts Generation

Human:

Given several sentences, break each of them into atomic facts with salient subject, relation, object. After splitting into atomic facts, we also rewrite the atomic fact to a (subject; relation; object) triple.
Here are some examples:

<example>
H:
Sentence 1: The Lunar Atmosphere and Dust Environment Explorer (LADEE) was a NASA lunar exploration and technology demonstration mission.

A:
<response>

For the first sentence: 

This part of sentence "The Lunar Atmosphere and Dust Environment Explorer (LADEE) was a NASA lunar exploration" can form one atomic fact:

The subject is "The Lunar Atmosphere and Dust Environment Explorer (LADEE)";
The relation is simply "was";
The object is "a NASA lunar exploration".
<sentence1-fact1>The Lunar Atmosphere and Dust Environment Explorer (LADEE) was a NASA lunar exploration</sentence1-fact1>
Into triple:
<sentence1-triple1>(The Lunar Atmosphere and Dust Environment Explorer (LADEE), was, a NASA lunar exploration)</sentence1-triple1>

This part of sentence "The Lunar Atmosphere and Dust Environment Explorer (LADEE) was technology demonstration mission" can form another fact:
The subject is "The Lunar Atmosphere and Dust Environment Explorer (LADEE)";
The relation is simply "was";
The object is "technology demonstration mission".
<sentence1-fact2>The Lunar Atmosphere and Dust Environment Explorer (LADEE) was technology demonstration mission</sentence1-fact2>
Into triple:
<sentence1-triple2>(The Lunar Atmosphere and Dust Environment Explorer (LADEE); was; technology demonstration mission)</sentence1-triple2>

</response>

</example>

Here is a new list of sentences. Please break each of them down into several facts as above.
{{sentence}}

Assistant:
\end{lstlisting}
\caption{Atomic Fact Breaking-down Prompt}
\label{fig:atomic_prompt}
\end{figure*}

==> prompts/coherence_check.tex <==
\begin{figure*}[htbp]
\begin{lstlisting}
## CoT coherence evaluation

Human:

Given a question, evaluate whether the thoughts support the provided answer for the question. Answer <support> or <not-support>.

Below are a few examples:

example 1:

Question: Is Ben Nevis taller than Snowdon?
Thoughts: Snowdon is 1,085 metres (3,560 ft) high. Ben Nevis is 1,345 metres (4,413 ft) high.
Answer: No
Support or not: Since the thoughts say Snowdon is 1,085 metres (3,560 ft) high. Ben Nevis is 1,345 metres (4,413 ft) high, then it means that Ben Nevis is taller than Snowdon. So the provided answer to the question is not supported by the thought. <not-support>

example 2:

Question: Is Ben Nevis taller than Snowdon?
Thoughts: Snowdon is 1,085 metres (3,560 ft) high. Ben Nevis is 1,345 metres (4,413 ft) high.
Answer: Yes
Support or not: Since the thoughts say Snowdon is 1,085 metres (3,560 ft) high. Ben Nevis is 1,345 metres (4,413 ft) high, then it means that Ben Nevis is taller than Snowdon. So the provided answer to the question is indeed supported by the thought. <support>

example 3:

Question: Is Houston located more west than Tampa?
Thoughts: Houston is located in the state of Texas. Tampa is located in the state of Florida. Florida is located in the southeastern United States. Texas is located in the central United States.
Answer: No
Support or not: Since the thoughts say Houston is in Texas and Texas in central US, while Tampa is in Florida and Florida is in southeastern US, then Texas is more west to Florida and thus Houston more west than Tampa. The provided answer is thus not supported by the thoughts. <not-support>


example 4:

Question: Is Houston located more west than Tampa?
Thoughts: Houston is located in the state of Texas. Tampa is located in the state of Florida. Florida is located in the southeastern United States. Texas is located in the central United States.
Answer: Yes
Support or not: Since the thoughts say Houston is in Texas and Texas in central US, while Tampa is in Florida and Florida is in southeastern US, then Texas is more west to Florida and thus Houston more west than Tampa. The provided answer is thus indeed supported by the thoughts. <support>

Here is a triple of new question, thought, answer:
Question: {}
{}

Please judge if the provided answer is supported using <support> or <not-support> to indicate.

Assistant:

\end{lstlisting}
\caption{Claude-based CoT coherence evaluation}
\label{fig:coherence_eval}
\end{figure*}

==> prompts/fact_generation.tex <==
\begin{figure*}[htbp]
\begin{lstlisting}
## Fact Generation

Human:

You are given a yes-no question. Your task is to answer the question by explicitly checking the relevant facts of the entities/events being compared in the question.

Here is one example:

Question: Is Mexico City more populous than Amsterdam?

Relevant facts related to <entity1>Mexico City</entity1>:
<facts_for_entity1>
<fact1>Mexico City has 22.2 million</fact1>
</facts_for_entity1>

Relevant facts related to <entity2>Amsterdam</entity2>:
<facts_for_entity2>
<fact1>Amsterdam has 821,752 in population </fact1>
</facts_for_entity2>

Now generate relevant fact for the following question.
{{question}}

Assistant:

\end{lstlisting}
\caption{Fact Generation Prompt}
\label{fig:fact_generation}
\end{figure*}


==> prompts/fact_verification.tex <==
\begin{figure*}[htbp]
\begin{lstlisting}
## Fact Verification 

Human:

You are given a sentence and you need to check whether it is consistent with the provided Wikipedia paragraphs.

Your task is to judge whether this sentence is factually consistent and potentially rewrite it. 

If inconsistent: rewrite the sentence by changing it minimally.
If consistent: leave it unchanged.

Here are four examples:

<example>

H:
Sentence: The Thermosphere, Ionosphere, Mesosphere Energetics and Dynamics (TIMED) satellite is a NASA mission.

Wikipedia paragraph: The TIMED (Thermosphere, Ionosphere, Mesosphere, Energetics and Dynamics) mission is dedicated to study the influences energetics and dynamics of the Sun and humans on the least explored and understood region of Earth's atmosphere: the Mesosphere and Lower Thermosphere / Ionosphere (MLTI). The mission was launched from Vandenberg Air Force Base in California on 7 December 2001 aboard a Delta II rocket launch vehicle. The project is sponsored and managed by NASA, while the spacecraft was designed and assembled by the Applied Physics Laboratory at Johns Hopkins University. The mission has been extended several times, and has now collected data over an entire solar cycle, which helps in its goal to differentiate the Sun's effects on the atmosphere from other effects. TIMED Was Launched Alongside Jason-1.

A:

<response>

Based on the paragraph, the sentence is factually consistent.
<factuality>Consistent</factuality>
Since it is consistent, we do not need to modify it.

</response>

</example>

Now, check the following sentence:
sentence: {{sentence}}

Wikipedia paragraph: {{retrieved paras}}

Assistant:
\end{lstlisting}
\caption{Fact Verification Prompt}
\label{fig:fact_verification}
\end{figure*}

==> prompts/recall_check.tex <==
\begin{figure*}[htbp]
\begin{lstlisting}
## fact recall evaluation

Human:

Given a paragraph and several facts, evaluate for each fact whether the information contained in the paragraph is consistent with it. For each fact, answer <consistent> or <inconsistent>. If the fact is completely unrelated to the paragraph, then ansewr <unrelated>.

Below are a few examples:

example 1:

Paragraph: Snowdon is 1,085 metres (3,560 ft) high. Ben Nevis is 1,345 metres (4,413 ft) high.
Fact: 
<1> The height of the summit as 1,085 m (3,560 ft), making Snowdon the highest mountain in Wales. </1>
<2> Ben Nevis is 2,000 meters high. </2>
<3> Mount Everest at 29,029 ft (8,848 m) is not only the highest peak in the Himalayas, but the highest peak on the entire planet. </3>

Evaluation: 
<1> The fact is talking about the height of the mountain Snowdon, and the paragraph mentions its height as well, thus the fact is related to the Paragraph. With regard to consistency, the paragraph says Snowdon is 1,085 metres (3,560 ft) high and the fact conveys the same thing, they are consistent. <consistent>. </1>

<2> The fact is talking about the height of the mountain Ben Nevis, and the paragraph mentions Ben Nevis's height, thus the fact is related. With regard to consistency, the paragraph says Ben Nevis is 1,345 metres (4,413 ft) high but the fact says it to be 2,000 meters high, which is very different, thus inconsistent. <inconsistent> </2>

<3> The fact is talking about the height of Mount Everest while the paragraph does not even mention Mount Everest, thus the fact is unrelated. <unrelated> </3>

example 2:

Paragraph: Houston is located in the state of Texas. Tampa is located in the state of Florida. Florida is located in the southeastern United States. Texas is located in the central United States.
Facts: 
<1> Houston is in Texas. </1>
<2> New York City is in the New York state. </2>
<3> Texas is in the middle of United States. </3>
<4> Florida is in the southeastern United States </4>

Evaluation: 
<1> The paragraph also mentions that Houston is in Texas, which is also indicated in this fact,thus it's both related and consistent. <consistent>. </1>

<2> The paragraph does not mention New York City or New York state. Thus it is not related. <unrelated> </2>

<3> The paragraph mentions that Texas is located in the central United States, which is indicated in the fact, thus the fact is consistent with the fact. <consistent> </3>

<4> The paragraph mentions that Florida is located in the southeastern United States, which is indicated in the fact, thus the fact is consistent with the fact. <consistent> </4>

Here is a paragraph and a list of facts:
Paragraph: {}
Facts: \n{}

Please judge if the fact and the paragraph is related. If related, indicate whether the fact is consistent with the paragraph using XML tags: <consistent> or <inconsistent>; If not, use the XML tag <unrelated> to indicate.

For each fact, Let's think step by step, following the above 2 examples.

Evaluation:

\end{lstlisting}
\caption{Claude-based fact recall evaluation}
\label{fig:fact_recall_eval}
\end{figure*}

==> prompts/support_check.tex <==

\begin{figure*}[htbp]
\begin{lstlisting}
## Data Filtering with Entailment Verification

Human:

You need to check whether given facts about multiple entities are consistent with the sentence. 
Here are a few examples:

<example>
H:
<question>Question: Who is the tallest guitarist?</question>
<answer>Marc Colombo</answer>
<fact>
Facts:

Marc Colombo: Marc Colombo is an American football player, not a guitarist.

Jimmy Page: Jimmy Page is an English musician who gained international fame for his work in the rock band Led Zeppelin. Jimmy Page has a height of 1.82 m or 5 feet 11.5 inches.

</fact>

A: 
<response>
The given facts state that Marc Colombo is an American football player, thus he cannot be the tallest guitarist. Thus these facts do not support the given answer to the question.
<consistency>No</consistency>
</response>
</example>

Here is a new pair of question-answer and facts. Please decide whether the given facts support the provided sentence:
<question>Question: {{question}}</question>
<answer>Answer: {{answer}}</answer>
<fact>Facts:
{{verified facts}}
</fact>

Assistant:
\end{lstlisting}
\caption{Data Filtering with Entailment Verification Prompt}
\label{fig:fact_filtering}
\end{figure*}

==> tables/fact_retrieval_results.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[scale=0.4]{figures/factrecallbar.png}
    \caption{Fact recall pre- and post-editing: measured by the relatedness and consistency of the decomposed atomic facts in CoT generation against the edited counterfactual facts. While both QLoRA and MEMIT maintains a reasonable degree of relatedness (with QLoRA outperforming MEMIT), there is a significant decline in factual consistency of both methods.}
    \label{fig:fact_retrieval}
\end{figure*}

% \begin{table*}[h]
%     \centering
%     \resizebox{16cm}{!}{
%     \begin{tabular}{lrrrrrrr}
%         \toprule
%          \multirow{2}{*}{\bf Scheme}& \multirow{2}{*}{\bf Model}&  \multicolumn{2}{c}{\bf Pre-edit}&  \multicolumn{2}{c}{\bf QLoRA}&  \multicolumn{2}{c}{\bf MEMIT}\\
%          \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
%          &  &  Relatedness&  Consistency&  Relatedness&  Consistency&  Relatedness& Consistency\\
%          \midrule
%          \multirow{2}{*}{superlative}&  7b&  52.79&  80.58&  53.88&  28.57&  39.62& 11.29\\
%          &  13b&  53.67&  81.89&  55.12&  28.61&  40.42& 10.75\\
%          \midrule
%          \multirow{2}{*}{comparative}&  7b&  85.43&  65.27&  79.16&  33.39&  40.08& 8.14\\
%          &  13b&  83.54&  63.89&  79.74&  28.49&  45.66& 15.73\\
%          \midrule
%          \multirow{2}{*}{counting}&  7b&  99.14&  43.92&  97.72&  9.89&  96.96& 4.56\\
%          &  13b&  99.64&  48.20&  98.02&  10.43&  97.08& 4.01\\
%          \midrule
%          \multirow{2}{*}{sorting}&  7b&  78.70&  60.50&  75.51&  46.67&  57.57& 53.04\\
%          &  13b&  77.74&  63.73&  78.05&  45.08&  59.70& 46.98\\
%          \midrule
%          \multirow{2}{*}{aggregation}&  7b&  62.61&  68.82&  86.40&  14.63&  79.13& 8.70\\
%          &  13b&  70.71&  76.91&  87.65&  11.85&  80.85& 5.97\\
%          \midrule
%          \multirow{2}{*}{subtraction}&  7b&  72.29&  70.67&  88.81&  15.00&  87.02& 7.86\\
%          &  13b&  77.57&  73.50&  90.93&  24.47&  87.24& 7.59\\
%          \midrule
%          \multirow{2}{*}{\it Average}&  7b&  75.16&  64.96&  80.25&  24.69&  66.73& 15.60\\
%          &  13b&  77.15&  68.02&  81.59&  24.82&  68.49& 15.17\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Fact recall pre- and post-editing: measured by the relatedness and consistency of the decomposed atomic facts in CoT generation against the edited counterfactual facts. While both QLoRA and MEMIT maintains a reasonable degree of relatedness (with QLoRA outperforming MEMIT), there is a significant decline in factual consistency of both methods.}
%     \label{tab:fact_retrieval}
% \end{table*}


